Distributed and Optimal Reduced Primal-Dual Algorithm for Uplink OFDM Resource Allocation

Orthogonal Frequency Division Multiplexing (OFDM) is the key component of many emerging broadband wireless access standards. The resource allocation in OFDM uplink, however, is challenging due to heterogeneity of users' Quality of Service requirements, channel conditions, and individual resource constraints. We formulate the resource allocation problem as a non-strictly convex optimization problem, which typically has multiple global optimal solutions. We then propose a reduced primal-dual algorithm, which is distributed, low in computational complexity, and probably globally convergent to a global optimal solution. The performance of the algorithm is studied through a realistic OFDM simulator. Compared with the previously proposed centralized optimal algorithm, our algorithm not only significantly reduces the message overhead but also requires less iterations to converge.

==> Conclusion.tex <==
\section{Conclusion and Future Work}
\label{sec:conclusions}

We presented the first distributed optimal primal-dual resource allocation
algorithm for uplink OFDM systems. The key features of the proposed
algorithm include: (a) incorporating practical OFDM system
constraints such as self-noise and maximum SNR constraints, (b)
reduced primal-dual algorithm which eliminates unnecessary variable
updates, (c) distributed implementation by the end users and base
station, (d) simple local updates with limited message passing, (e)
global convergence despite of the existence of multiple global
optimal solutions, and (f) fast convergence compared with the
state-of-art centralized optimal algorithm. Currently we are
extending this work in several directions, including proving the
theoretical convergence speed of the algorithm.

%\section*{Acknowledgement}
%%We want to thank R.~Agrawal, R.~Berry and V.~Subramanian for helpful discussions.
%We want to acknowledge helpful discussions with Professor Randall Berry from Northwestern University, Dr. Vijay G. Subramanian from National %University of Ireland, and Dr. Rajeev Agrawal from Motorola Inc.

